RoCode: A Dataset for Measuring Code Intelligence from Problem Definitions in Romanian

Recently, large language models (LLMs) have become increasingly powerful and have become capable of solving a plethora of tasks through proper instructions in natural language. However, the vast majority of testing suites assume that the instructions are written in English, the de facto prompting language. Code intelligence and problem solving still remain a difficult task, even for the most advanced LLMs. Currently, there are no datasets to measure the generalization power for code-generation models in a language other than English. In this work, we present RoCode, a competitive programming dataset, consisting of 2,642 problems written in Romanian, 11k solutions in C, C++ and Python and comprehensive testing suites for each problem. The purpose of RoCode is to provide a benchmark for evaluating the code intelligence of language models trained on Romanian / multilingual text as well as a fine-tuning set for pretrained Romanian models. Through our results and review of related works, we argue for the need to develop code models for languages other than English.

==> table/code-switching.tex <==
\begin{table}[hbt!]
    \begin{tabular}{l}
         \begin{tcolorbox}[
            enhanced,
            attach boxed title to top left={xshift=6mm,yshift=-3mm},
            colback=lightgreen!20,
            colframe=lightgreen,
            colbacktitle=lightgreen,
            title={\scriptsize Code-Code-Switching in Solutions},
            fonttitle=\bfseries\color{black},
            boxed title style={size=small,colframe=lightgreen,sharp corners},
            sharp corners,
        ]
{\scriptsize
        \begin{minted}{cpp}
int main(void)
{
    // a.k.a. "read"
    citire(); 
    nr = 0;
    // a.k.a "number of steps"
    max = nr_pasi(max); 
    radx(max, w, n);
        
    // a.k.a. "solve"
    rezolvare(); 
        
    // a.k.a. "print"
    printare(); 
    return 0;
}
\end{minted}
}
\end{tcolorbox}
    \end{tabular}
    \caption{Example of a snippet from a C / C++ solution that exhibits code-code-switching: function names / variables are written in Romanian, whereas language keywords are written in English. Comments added by the paper authors.}
    \label{tab:code-code-switching}
\end{table}

==> table/romanian-results.tex <==
\begin{table}[hbt!]
    \centering
    \resizebox{\linewidth}{!}{
    \begin{tabular}{lc|cc|cc}
        \textbf{Model} & \textbf{\# Params} & \textbf{Accuracy} &  \textbf{Strict Accuracy} & \textbf{pass@1} & \textbf{pass@10} \\ 
        \midrule
        RoGPT2-base & 124M & 0.0 & 0.0 & 0.0 & 0.0 \\
        RoGPT2-medium & 354M & 0.0 & 0.0 & 0.0 & 0.0 \\
        RoGPT2-large & 774M & 0.0 & 0.0 & 0.0 & 0.0 \\
        GPT-Neo-Ro & 780M & 0.0 & 0.0 & 0.0 & 0.0 \\
    \end{tabular}}
    \caption{Results on RoCode for available Romanian models. \textbf{None} of the currently available Romanian language models are able to understand the problem definition or to produce code.}
    \label{tab:ro-results}
\end{table}
